Geometry of Resource Interaction - A Minimalist Approach

The Resource $\lambda$-calculus is a variation of the $\lambda$-calculus where arguments can be superposed and must be linearly used. Hence it is a model for linear and non-deterministic programming languages, and the target language of Ehrhard-Taylor expansion of $\lambda$-terms. In a strictly typed restriction of the Resource $\lambda$-calculus, we study the notion of path persistence, and we define a Geometry of Interaction that characterises it, is invariant under reduction, and counts addends in normal forms.

==> eptcsdata.tex <==
\providecommand{\firstpage}{79}
\providecommand{\publicationstatus}{S. Alves and I. Cervesato (Eds): Third International Workshop\\ on Linearity 2014 (LINEARITY'14)\\
EPTCS 176, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.176.7}{10.4204/EPTCS.176.7}}
\pdfoutput=1

